$L^p$- Partially null controllability of abstract fractional differential inclusion with nonlocal condition

In this work, we investigate the $L^p$- partial null controllability of the abstract semilinear fractional-order differential inclusion with nonlocal conditions. The set of admissible controls is characterized by $u\in L^p(I,U)$, $1<p<\infty$, $I=[0,\nu]$, where $U$ is a uniformly convex Banach space. Assuming partial null controllability for the fractional-order linear system with a source term, we employ an approximate solvability method to simplify the problem to reduce it to finite-dimensional subspaces. Consequently, the solutions of the original problem are obtained as limiting functions within these subspaces. The paper tackles a challenge stemming from the assumption that $U$ is a uniformly convex Banach space, which introduces convexity issues in constructing the required control. These complications do not occur if $U$ is a separable Hilbert space. This study introduces a novel approach by resolving the convexity issue, thereby enabling $L^p(I, U)$ partially null controllability of the semilinear fractional-order differential control system, with $U$ being a uniformly convex Banach space.

==> sn-bibliography <==
@article {MR3278850,
    AUTHOR = {Benedetti, Irene and Obukhovskii, Valeri and Taddei,
              Valentina},
     TITLE = {Controllability for systems governed by semilinear evolution
              inclusions without compactness},
   JOURNAL = {NoDEA Nonlinear Differential Equations Appl.},
  FJOURNAL = {NoDEA. Nonlinear Differential Equations and Applications},
    VOLUME = {21},
      YEAR = {2014},
    NUMBER = {6},
     PAGES = {795--812},
      ISSN = {1021-9722},
   MRCLASS = {93B05 (28B20 34G25 47H04)},
  MRNUMBER = {3278850},
MRREVIEWER = {G. Anichini},
       DOI = {10.1007/s00030-014-0267-0},
       URL = {https://doi.org/10.1007/s00030-014-0267-0},
}
@article {MR2953606,
    AUTHOR = {Benedetti, Irene and Obukhovskii, Valeri and Zecca, Pietro},
     TITLE = {Controllability for impulsive semilinear functional
              differential inclusions with a non-compact evolution operator},
   JOURNAL = {Discuss. Math. Differ. Incl. Control Optim.},
  FJOURNAL = {Discussiones Mathematicae. Differential Inclusions, Control
              and Optimization},
    VOLUME = {31},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {39--69},
      ISSN = {1509-9407},
   MRCLASS = {93B05 (34G25 34K45 47H08)},
  MRNUMBER = {2953606},
MRREVIEWER = {Jos\'{e} Alberto Murillo Hern\'{a}ndez},
       DOI = {10.7151/dmdico.1127},
       URL = {https://doi.org/10.7151/dmdico.1127},
}
@article {MR2503088,
    AUTHOR = {Obukhovski, Valeri and Zecca, Pietro},
     TITLE = {Controllability for systems governed by semilinear
              differential inclusions in a {B}anach space with a noncompact
              semigroup},
   JOURNAL = {Nonlinear Anal.},
  FJOURNAL = {Nonlinear Analysis. Theory, Methods \& Applications. An
              International Multidisciplinary Journal},
    VOLUME = {70},
      YEAR = {2009},
    NUMBER = {9},
     PAGES = {3424--3436},
      ISSN = {0362-546X},
   MRCLASS = {93B05 (34A60 34G25 47H20 47N70 49J20)},
  MRNUMBER = {2503088},
MRREVIEWER = {Lianwen Wang},
       DOI = {10.1016/j.na.2008.05.009},
       URL = {https://doi.org/10.1016/j.na.2008.05.009},
}
@article {MR4475865,
    AUTHOR = {Malaguti, Luisa and Perrotta, Stefania and Taddei, Valentina},
     TITLE = {{$L^p$}-exact controllability of partial differential
              equations with nonlocal terms},
   JOURNAL = {Evol. Equ. Control Theory},
  FJOURNAL = {Evolution Equations and Control Theory},
    VOLUME = {11},
      YEAR = {2022},
    NUMBER = {5},
     PAGES = {1533--1564},
      ISSN = {2163-2472},
   MRCLASS = {93B07 (34B10 93C25)},
  MRNUMBER = {4475865},
MRREVIEWER = {Akram Ben Aissa},
       DOI = {10.3934/eect.2021053},
       URL = {https://doi.org/10.3934/eect.2021053},
}
@article {MR3750671,
    AUTHOR = {Zhou, Yong and Peng, Li and Ahmad, Bashir},
     TITLE = {Topological properties of solution sets for stochastic
              evolution inclusions},
   JOURNAL = {Stoch. Anal. Appl.},
  FJOURNAL = {Stochastic Analysis and Applications},
    VOLUME = {36},
      YEAR = {2018},
    NUMBER = {1},
     PAGES = {114--137},
      ISSN = {0736-2994,1532-9356},
   MRCLASS = {34G25 (34F05 35R60 37L55 60H10 60H15)},
  MRNUMBER = {3750671},
MRREVIEWER = {Ezekiel\ O.\ Ayoola},
       DOI = {10.1080/07362994.2017.1374191},
       URL = {https://doi.org/10.1080/07362994.2017.1374191},
}
@article {MR1784435,
    AUTHOR = {Brze\'zniak, Zdzis\l aw and Elworthy, K. D.},
     TITLE = {Stochastic differential equations on {B}anach manifolds},
   JOURNAL = {Methods Funct. Anal. Topology},
  FJOURNAL = {Methods of Functional Analysis and Topology},
    VOLUME = {6},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {43--84},
      ISSN = {1029-3531,2415-7503},
   MRCLASS = {58J65 (46E35 46G12 58B99 60H10)},
  MRNUMBER = {1784435},
MRREVIEWER = {Ya.\ \=I.\ B\=\i lopol\cprime s\cprime ka},
}
@article {MR3634281,
    AUTHOR = {Zhu, Jiahui and Brze\'zniak, Zdzis\l aw and Hausenblas, Erika},
     TITLE = {Maximal inequalities for stochastic convolutions driven by
              compensated {P}oisson random measures in {B}anach spaces},
   JOURNAL = {Ann. Inst. Henri Poincar\'e{} Probab. Stat.},
  FJOURNAL = {Annales de l'Institut Henri Poincar\'e{} Probabilit\'es et
              Statistiques},
    VOLUME = {53},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {937--956},
      ISSN = {0246-0203,1778-7017},
   MRCLASS = {60H15 (60F10 60G57 60H05 60J75)},
  MRNUMBER = {3634281},
       DOI = {10.1214/16-AIHP743},
       URL = {https://doi.org/10.1214/16-AIHP743},
}
@article {MR1402663,
    AUTHOR = {Peng, Shi-Ge},
     TITLE = {Backward stochastic differential equation and exact
              controllability of stochastic control systems},
   JOURNAL = {Progr. Natur. Sci. (English Ed.)},
  FJOURNAL = {Progress in Natural Science. English Edition},
    VOLUME = {4},
      YEAR = {1994},
    NUMBER = {3},
     PAGES = {274--284},
      ISSN = {1002-0071,1745-5391},
   MRCLASS = {93E03 (34F05 60H10 93B05)},
  MRNUMBER = {1402663},
MRREVIEWER = {Igor\ N.\ Litvin},
}
@article {MR216893,
    AUTHOR = {Connors, Michael M.},
     TITLE = {Controllability of discrete, linear, random dynamical systems},
   JOURNAL = {SIAM J. Control},
  FJOURNAL = {SIAM J. Control},
    VOLUME = {5},
      YEAR = {1967},
     PAGES = {183--210},
   MRCLASS = {93.60},
  MRNUMBER = {216893},
MRREVIEWER = {P.\ E.\ Sarachik},
}
@article {MR2841348,
    AUTHOR = {Shi, Yan Cheng and Zhou, Yuan},
     TITLE = {Controllability of linear stochastic control systems},
   JOURNAL = {J. Fudan Univ. Nat. Sci.},
  FJOURNAL = {Fudan University. Journal. Natural Science. Fudan Xuebao.
              Ziran Kexue Ban},
    VOLUME = {50},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {31--38},
      ISSN = {0427-7104},
   MRCLASS = {93B05 (60G35 60H10 93E03)},
  MRNUMBER = {2841348},
}
@article {MR398595,
    AUTHOR = {Sunahara, Yoshifumi and Aihara, Shin'ichi and Kishino,
              Kiyotaka},
     TITLE = {On the stochastic observability and controllability non-linear
              systems},
   JOURNAL = {Internat. J. Control},
  FJOURNAL = {International Journal of Control},
    VOLUME = {22},
      YEAR = {1975},
    NUMBER = {1},
     PAGES = {65--82},
      ISSN = {0020-7179,1366-5820},
   MRCLASS = {93B05 (93E10)},
  MRNUMBER = {398595},
MRREVIEWER = {R.\ Rishel},
       DOI = {10.1080/00207177508922061},
       URL = {https://doi.org/10.1080/00207177508922061},
}
@article {MR1833025,
    AUTHOR = {Mahmudov, Nazim Idrisoglu},
     TITLE = {Controllability of linear stochastic systems},
   JOURNAL = {IEEE Trans. Automat. Control},
  FJOURNAL = {Institute of Electrical and Electronics Engineers.
              Transactions on Automatic Control},
    VOLUME = {46},
      YEAR = {2001},
    NUMBER = {5},
     PAGES = {724--731},
      ISSN = {0018-9286,1558-2523},
   MRCLASS = {93B05 (93E03)},
  MRNUMBER = {1833025},
MRREVIEWER = {N.\ U.\ Ahmed},
       DOI = {10.1109/9.920790},
       URL = {https://doi.org/10.1109/9.920790},
}
@book {MR454768,
    AUTHOR = {Fleming, Wendell H. and Rishel, Raymond W.},
     TITLE = {Deterministic and stochastic optimal control},
    SERIES = {Applications of Mathematics},
    VOLUME = {No. 1},
 PUBLISHER = {Springer-Verlag, Berlin-New York},
      YEAR = {1975},
     PAGES = {vii+222},
   MRCLASS = {49-02 (93-02)},
  MRNUMBER = {454768},
MRREVIEWER = {H.\ J.\ Kushner},
}
@article {MR3932620,
    AUTHOR = {Dou, Fangfang and Lu, Qi},
     TITLE = {Partial approximate controllability for linear stochastic
              control systems},
   JOURNAL = {SIAM J. Control Optim.},
  FJOURNAL = {SIAM Journal on Control and Optimization},
    VOLUME = {57},
      YEAR = {2019},
    NUMBER = {2},
     PAGES = {1209--1229},
      ISSN = {0363-0129,1095-7138},
   MRCLASS = {93B05 (60H15 93E03)},
  MRNUMBER = {3932620},
MRREVIEWER = {Abdulrahman\ S.\ Al-Hussein},
       DOI = {10.1137/18M1164640},
       URL = {https://doi.org/10.1137/18M1164640},
}
@article {MR3629137,
    AUTHOR = {Zhou, Yong and Peng, Li and Ahmad, Bashir and Alsaedi, Ahmed},
     TITLE = {Topological properties of solution sets of fractional
              stochastic evolution inclusions},
   JOURNAL = {Adv. Difference Equ.},
  FJOURNAL = {Advances in Difference Equations},
      YEAR = {2017},
     PAGES = {Paper No. 90, 20},
      ISSN = {1687-1839,1687-1847},
   MRCLASS = {34G25 (26A33 34F05 34K37 37L55 60H15)},
  MRNUMBER = {3629137},
MRREVIEWER = {Selvaraj\ Suganya},
       DOI = {10.1186/s13662-017-1142-1},
       URL = {https://doi.org/10.1186/s13662-017-1142-1},
}
@book {MR4363403,
    AUTHOR = {L\"u, Qi and Zhang, Xu},
     TITLE = {Mathematical control theory for stochastic partial
              differential equations},
    SERIES = {Probability Theory and Stochastic Modelling},
    VOLUME = {101},
 PUBLISHER = {Springer, Cham},
      YEAR = {[2021] \copyright 2021},
     PAGES = {xiii+592},
      ISBN = {978-3-030-82330-6; 978-3-030-82331-3},
   MRCLASS = {93-02 (60H15 60H30 93B05 93C20)},
  MRNUMBER = {4363403},
MRREVIEWER = {Ramalingam\ Udhayakumar},
       DOI = {10.1007/978-3-030-82331-3},
       URL = {https://doi.org/10.1007/978-3-030-82331-3},
}
@article{zhang2021analysis,
  title={Analysis of stochastic process to model safety risk in construction industry},
  author={Zhang, Zhenhao and Li, Wenbiao and Yang, Jianyu},
  journal={Journal of Civil Engineering and Management},
  volume={27},
  number={2},
  pages={87--99},
  year={2021}
}
@article{fischer2019electric,
  title={Electric vehicles’ impacts on residential electric local profiles--A stochastic modelling approach considering socio-economic, behavioural and spatial factors},
  author={Fischer, David and Harbrecht, Alexander and Surmann, Arne and McKenna, Russell},
  journal={Applied energy},
  volume={233},
  pages={644--658},
  year={2019},
  publisher={Elsevier}
}
@article{omar2021fractional,
  title={Fractional stochastic models for COVID-19: Case study of Egypt},
  author={Omar, Othman AM and Elbarkouky, Reda A and Ahmed, Hamdy M},
  journal={Results in Physics},
  volume={23},
  pages={104018},
  year={2021},
  publisher={Elsevier}
}
@article{guido2020feasibility,
  title={Feasibility of stochastic models for evaluation of potential factors for safety: a case study in Southern Italy},
  author={Guido, Giuseppe and Haghshenas, Sina Shaffiee and Haghshenas, Sami Shaffiee and Vitale, Alessandro and Astarita, Vittorio and Haghshenas, Ashkan Shafiee},
  journal={Sustainability},
  volume={12},
  number={18},
  pages={7541},
  year={2020},
  publisher={MDPI}
}
article{fuentes2002algunos,
  title={Algunos aspectos matem{\'a}ticos del problema del reparto de secretos},
  author={Fuentes, P Abascal},
  journal={SeMA Journal: Bolet{\'\i}n de la Sociedad Espa{\~n}ola de Matem{\'a}tica Aplicada},
  number={21},
  pages={51--64},
  year={2002},
  publisher={Sociedad Espa{\~n}ola de Matem{\'a}tica Aplicada}
}
@book{li2012optimal,
  title={Optimal control theory for infinite dimensional systems},
  author={Li, Xungjing and Yong, Jiongmin},
  year={2012},
  publisher={Springer Science \& Business Media}
}
@phdthesis{tiberio2004stochastic,
  title={Stochastic and deterministic differential equation modeling: The accuracy of recovering dynamic model parameters of change},
  author={Tiberio, Stacey S},
  year={2004},
  school={University of Notre Dame}
}
@article {MR2984588,
    AUTHOR = {L\"u, Qi and Yong, Jiongmin and Zhang, Xu},
     TITLE = {Representation of {I}t\^o{} integrals by {L}ebesgue/{B}ochner
              integrals},
   JOURNAL = {J. Eur. Math. Soc. (JEMS)},
  FJOURNAL = {Journal of the European Mathematical Society (JEMS)},
    VOLUME = {14},
      YEAR = {2012},
    NUMBER = {6},
     PAGES = {1795--1823},
      ISSN = {1435-9855,1435-9863},
   MRCLASS = {60H25 (46G12 60B11 60G05 60G07 60H05 91B24)},
  MRNUMBER = {2984588},
MRREVIEWER = {Markus\ Riedle},
       DOI = {10.4171/JEMS/347},
       URL = {https://doi.org/10.4171/JEMS/347},
}
